Planck intermediate results. XLII. Large-scale Galactic magnetic fields

Recent models for the large-scale Galactic magnetic fields in the literature have been largely constrained by synchrotron emission and Faraday rotation measures. We use three different but representative models to compare their predicted polarized synchrotron and dust emission with that measured by the Planck satellite. We first update these models to match the Planck synchrotron products using a common model for the cosmic-ray leptons. We discuss the impact on this analysis of the ongoing problems of component separation in the Planck microwave bands and of the uncertain cosmic-ray spectrum. In particular, the inferred degree of ordering in the magnetic fields is sensitive to these systematic uncertainties, and we further show the importance of considering the expected variations in the observables in addition to their mean morphology. We then compare the resulting simulated emission to the observed dust polarization and find that the dust predictions do not match the morphology in the Planck data but underpredict the dust polarization away from the plane. We modify one of the models to roughly match both observables at high latitudes by increasing the field ordering in the thin disc near the observer. Though this specific analysis is dependent on the component separation issues, we present the improved model as a proof of concept for how these studies can be advanced in future using complementary information from ongoing and planned observational projects.

==> synchrotron_features.tex <==

\addedC{In this Appendix, we discuss qualitatively some of the individual features seen in the comparison of the models with the data.}

\subsection{The Fan region}

The amplitude of the Perseus arm can be adjusted to match some of the
emission in the Fan region in the second quadrant.  But there remains
residual total intensity emission visible in the maps to differing
degrees depending on the field model, and a strong emission peak in
polarized synchrotron, at roughly $\ell\approx160\degr$.  None of
the models have a peak in that direction.  Furthermore, increasing the
amplitude of that arm to match the peak in the second quadrant
polarization would overpredict in the third quadrant significantly.  Therefore,
these models still cannot explain the Fan region.  There remains excess
emission that does not follow the prediction of a spiral arm in the
outer Galaxy with a pitch angle similar to what we have used.

All the models have roughly the same pitch angle of around $-12\degr$,
and though this matches some of the RM data along the plane and 
the pitch angle of the material spiral pattern, it is highly
uncertain.  A pitch angle of $\theta<-12\degr$, i.e., an angle
that means the arms open faster, could shift the model's peak emission
in the outer Galaxy towards lower longitudes.  But whatever the pitch
angle, the emission peak would not likely be as well-defined as the observed
morphology; it would remain a broad modulation, as in the current
models, simply shifted.  It is therefore unlikely that the Fan region
is the result of the large-scale geometry such as the spiral arms.
  
In Fig.\,\ref{fig:chisq_maps_synch}, we see that above the plane,
all models underpredict the emission from the Fan.  (This is
exaggerated in the {\jf}b model because of the anti-symmetry in the
halo component discussed below.)  \added{Furthermore, as can be seen
  in \citet{wolleben:2006}, this region stands out in polarization at
  radio frequencies as a thick feature extending up to
  $b\approx20\degr$ despite the fact that all of the rest of the
  Galactic plane region is depolarized by Faraday effects.  This
  large-scale morphology argues for its origin as a relatively local
  emission region, but the question of its nature remains open.}
 


\subsection{Inner versus outer Galaxy}

The models were updated to try to match the latitude profiles in the
inner Galaxy and the longitude profiles in the Galactic plane.  The
latitude profiles in the outer Galaxy, however, do not agree well.
Some of this is due to the Fan region in the second quadrant, so to
look at the outer Galaxy latitude profile in
Fig.\,\ref{fig:lat_prof_comp_synch}, we only use the third quadrant.

For the Jansson12 models, the anti-symmetry in the Faraday RMs is reproduced by a reversal in the halo
component in the north as compared to the south.  This in turn
partially cancels the disc field near their transition region (at a
few hundred pc in height) and causes a visible asymmetry in the
synchrotron emission that is particularly apparent in the outer
Galaxy at intermediate latitudes (bottom panel of
Fig.\,\ref{fig:lat_prof_comp_synch}) and does not match the data.  We
have focused on the inner two quadrants where the observations cover
most of the Galactic disc and have left this mismatch in the outer
Galaxy.  It could in principle be reduced by introducing further
complexity to the model in the Perseus arm and in the radial dependence of
the disc height parameters, or by removing this anti-symmetry in the
halo component across the Galactic plane.



\subsection{Spiral arms}

One change to the {\jf} model in the inner Galaxy can be seen in the
features along the Galactic plane just to each side of the Galactic
centre.  At $\ell\approx30\degr$, the modelled polarization is dominated
by the Perseus arm on the far side.  The $\ell\approx-30\degr$ area is
dominated by the near side of the Scutum arm and to a lesser degree
includes a contribution from the Perseus arm on the far side.  
%The
%updated {\jf} model has a lower Perseus arm amplitude than the
%original.  So though the original model is \added{brighter at $10\degr\le \ell
%\le 40\degr$, the update is brighter} on the negative side.  
\added{But it is important to realize that these
  regions do not tell us much about the spiral
  arms.  On the positive longitude side, there is a dip in the the polarized
synchrotron emission}, and as mentioned above, this may be due to
polarization cancellation from the NPS crossing the plane.
Furthermore, the emission on the
negative longitude side has the largest uncertainty due to systematics.  The
data therefore do not provide strong constraints on the arms in this
region.  Instead, the change in the model was driven by the global amount
of emission in the outer versus inner Galaxy, \added{ and the changes in these
inner Galaxy features are not well constrained}.  

The updated Jaffe13b model is not as good a fit to the data, which
again is unsurprising given that the original model was constrained
relative to the data with an MCMC optimization.  A repeat of that
analysis in the plane would improve the morphological match \added{by
  adjusting the positions and amplitudes of the arm ridges in each
  field component, since it is the tangents to these ridges that create the shoulder-like features
  in the longitude profile}.  In
particular, the spiral arm tangents, seen as shoulders in the
longitude profile in Fig.\,\ref{fig:lon_prof_comp_synch}, do not match
as well, indicating a need to adjust the locations of
the spiral arms.  


\subsection{X-shaped halo magnetic field}


%\input{jf_x}

%Figure\,\ref{fig:jf_x} explicitly compares the {\em original} {\jf} model with and
%without the x-shaped field component for the polarization observables.
%The effect of the x-shaped field on the morphology is clear towards the
%inner galaxy for all but the highest latitudes ($|b|\gsim60\degr$).
%It seems to match the morphology of the Stokes $Q$ above the Galactic
%plane.  Below the plane, the correspondence is significantly less
%clear.  For Stokes $U$, the inner Galaxy above and below the plane
%match the x-shaped model better.  In both observables, the outer
%Galaxy below the plane is wrong.

In the updated {\jf}b model, the x-shaped field is reduced
significantly in order not to overpredict the high-latitude
synchrotron polarization.  This is degenerate, however, with other
parameters such as the amplitudes of the toroidal halo components.

Though the {\jf} analysis masked out the bright limb of the NPS, it is
unclear how much of the sky towards the inner Galaxy is related.  The
loop appears to continue below the Galactic plane;  see, e.g., the
discussion in \citet{planck2014-a31}.  Such large-scale structures
perturb the polarization to an unknown degree at high latitudes.  It
is therefore very difficult to characterize the robustness of the
claimed detection of the x-shaped field.  An independent tracer of
such fields will likely be necessary (see, e.g., \citealt{west:2016}).  

In the {\jf} field model, the toroidal field component is zeroed in the
Galactic plane,
leaving only the disc component made of \addedB{spiral} segments and the x-shaped
field component.  The x-shaped component then has a large effect on
the amount of emission in the plane towards the inner Galaxy.  Since it
appears largely perpendicular to the disc component when projected
onto the sky, the two components tend to cancel each other \added{in the inner plane.
This makes any fitting sensitive here to their relative amplitudes in
a way that is unlikely to be physically realistic.}  The Galactic plane was
masked in the original {\jf} synchrotron analysis, so it was not affected by
this aspect of the x-shaped field implementation.  This implies that
the current parametrization is not ideal for exploring the likelihood
space for the x-shaped field component amplitude when integrating
through the whole disc in synchrotron and dust emission.




